6LoRa: Full Stack IPv6 Networking with DSME-LoRa on Low Power IoT Nodes

Long range wireless transmission techniques such as LoRa are preferential candidates for a substantial class of IoT applications, as they avoid the complexity of multi-hop wireless forwarding. The existing network solutions for LoRa, however, are not suitable for peer-to-peer communication, which is a key requirement for many IoT applications. In this work, we propose a networking system - 6LoRa, that enables IPv6 communication over LoRa. We present a full stack system implementation on RIOT OS and evaluate the system on a real testbed using realistic application scenarios with CoAP. Our findings confirm that our approach outperforms existing solutions in terms of transmission delay and packet reception ratio at comparable energy consumption.

==> figures/colors_common.tex <==
\definecolor{opendsme}{RGB}{255,255,179}
\definecolor{flora}{RGB}{141,211,199}
\definecolor{inet}{RGB}{190,186,218}
\definecolor{own}{RGB}{251,128,114}

==> tex/discussion.tex <==
\section{Design discussions}\label{sec:discussion}

In this section, we comparatively discuss SCHC over LoRaWAN and
6LoWPAN over DSME-LoRa, and deepen the analysis of their performances. We also propose mappings for different application use
cases based on our previous performance evaluation of both protocols. The
findings demonstrate that our proposed solution yields superior packet
reception rate and shorter completion times compared to SCHC over LoRaWAN for
end-to-end device communication in the proposed peer-to-peer network.

The downlink communication in LoRaWAN imposes a significant burden on the
network, as the gateways are unable to receive data from devices while
transmitting. Furthermore, the LoRaWAN network server relies on the MAC
schedule of the devices and gateways to accommodate downlink transmissions,
resulting in unreliable and non-deterministic packet reception. While the
impact of adding more gateways on peer-to-peer communication in LoRaWAN has not
been evaluated, it is worth noting that this solution can mitigate the problem
in three ways: (i) by increasing the packet reception rate of uplink packets due
to the capture effect of the LoRa modulation, (ii) by reducing packet losses due to gateways
receiving uplinks while transmitting, and (iii) by increasing the downlink
bandwidth. 

Deploying more gateways will increase network cost and 
complexity. Alternatively, sensor devices may transmit using different
spreading factor settings to enhance the uplink packet reception rate, but this
approach does not address the issue concerning downlink communication.
For these reasons, DSME-LoRa is the preferred choice for the transmission of critical or real-time data in peer-to-peer scenarios.

The packet reception rate of
DSME-LoRa does not depend on the number of devices or the network topology~\cite{aksw-dslrc-22}.
Nevertheless, these settings may affect the completion time of end-to-end
communication due to GTS scheduling. For example,
increasing the superframe duration in a star topology to support the allocation
of one slot for each transmitting device may lead to increased completion time. On the
other hand, devices in a mesh topology can transmit data concurrently in 
guaranteed time slots, reducing the number of required slots and superframe duration, which decreases 
completion time. Therefore, SCHC over LoRaWAN is the
preferred choice for star topologies.

It has been observed that SCHC over LoRaWAN demands fewer memory resources
compared to 6LoWPAN over LoRaWAN. It is noteworthy, though, that both
solutions are capable of operating in devices that fall under the category of
class 2 constrained devices~\cite{RFC-7228} ($\approx$256\,kB RAM and $\approx$50\,kB of RAM).

In the context of low-power devices, it has been observed that LoRaWAN offers
superior energy efficiency as compared to DSME-LoRa, making it the preferred
option for transmitting non-critical data. However, for critical traffic,
DSME-LoRa can still operate on low-power while facilitating the transmission
and reception of data. Nevertheless, it is worth noting that sleepy DSME-LoRa
end devices are unable to receive multicast packets due to the inactivity of
the transceiver during the contention access period. For applications that
depend on multicast traffic, LoRaWAN operating in Class B (which has not been
evaluated) may be a more suitable alternative.

% Compression ratio
Our evaluation indicates that the compression ratio of SCHC is higher
than that of 6LoWPAN. This is attributed due to the lower protocol overhead of SCHC,
which involves only one byte for the Rule ID encoded in the FPort fields of the LoRaWAN
packet, and its capability to compress additional header fields such as the entire
UDP header. Furthermore, SCHC can compress the CoAP header, which is not possible with 6LoWPAN.
These findings serve as a driving force for further exploration of SCHC over IEEE 802.15.4,
which is currently under discussion in the IETF.


==> tex/model.tex <==
\section{Extended analytical Markov model}\label{sec:model}

\begin{figure*}
    \centering
    \input{figures/model}
    \caption{Model estimation of the transmission delay distribution for varying system utilization (\%) and number of slots. We define the system utilization as the percentage
    of the multisuperframe duration over the transmission interval and assume the multisuperframe duration is 3.84\,s.}
    \label{fig:model}
\end{figure*}

DSME-LoRa can be configured with bounded waiting times, which we derived via 
an analytical stochastic model %\cite{aksw-dslrc-22} 
\todo{anonymous}.
To guarantee an optimal GTS schedule for the CoAP Observe mechanism, we extend 
this model to accommodate multiple guaranteed time slots which target at 
 a single neighbour.


The original model assumes exponentially distributed interarrival times for
packet scheduling and utilizes an ergodic Markov chain to estimate the queue
length distribution at the end of each slot, which leads to the calculation of
the queue length at an arbitrary time. For our new model, we consider a
multisuperframe with N TX slots to the same target device. The calculation of
the exact queue length distribution is involved and depends on the location of
each slot. Therefore we simplify the model by assuming a single slot can
transmit up to N frames simultaneously.


Let A be the number of scheduled frames during a multisuperframe. The
Markov transition arcs, which describe the transition probability from
$i$ queued frames at the beginning of the multisuperframe to $j$ frames at
the beginning of the next multisuperframe, are defined by:

\begin{numcases}{P[i,j] =}
    P(A \leq N-i) & \text{if} j = 0 \label{eq:m1}\\
    P(A = j-i+N) & \text{otherwise}  \label{eq:m2}
\end{numcases}

\autoref{eq:m1} describes the probability of empty MAC queue at the beginning of
the next multisuperframe, given $i$ queued frames at the beginning of current the multisuperframe.
This occurs when the sum of queued frames and the number of schedule packets during the multisuperframe
does not exceed the number of allocated slots. \autoref{eq:m2} describes the
probability of $j$ queued frames in the beginning of the next multisuperframe,
given $i$ queued frames at the beginning of the current multisuperframe.

%\cite{aksw-dslrc-22} 
\todo{anonymous} proves that the number of frames scheduled between the
last slot and an arbitrary time evaluates to $P(N(t-S,S)=j) = \frac{1}{\rho} \cdot \Gamma(j+1,\rho)$,
with $\rho$ the system utilization ($\rho = \lambda \cdot T_{msf}$,  $\lambda$ is the transmission schedule rate, $T_{msf}$ the duration of a multisuperframe,  and $\Gamma(j+1,\rho)$ the regularized lower incomplete gamma function).

Analogously, the distribution of queue entries $L(t)$ at an arbitrary time $t$ reads   
\begin{equation}
P\{L(t) = j\} = \sum_{i=0}^{j} \pi_{j-i} \frac{\Gamma(i+1,\rho)}{\rho},
\end{equation}
with
$\pi_i$ the stationary distribution of the Markov chain, which exists if the
system utilization per slot is less than a unit ($\frac{\rho}{N} < 1$).
The equation uses the
law of total probability to calculate the probability of $j$ packets in the queue,
given the stationary distribution of $i$ packets in the queue at the beginning
of the multisuperframe is known.

Following a similar approach from the original model, the distribution of transmission delay in
multiples of $T_{msf}$ derives to:
\begin{equation}
	P\{W \leq n \cdot T_{msf}\} = P\{L(t) \leq N \cdot n - 1\}
\end{equation}

This result reflects that the transmission of $N \cdot n$ frames takes at most $n$ multisuperframes
and therefore the packet in position $N$  of the queue (scheduled when there
are $N-1$ queued packets) takes at most $n$ multisuperframes.



\autoref{fig:model} depicts the model estimation of transmission delays under varying
system utilization and numbers of allocated slots. For low system utilization
(left) increasing the number of slots shows small variations in transmission delay,
because of low queue stress in the single slot scenario (N=1). For high system
utilization (right), the stress in the MAC queue is high for the single slot
scenario (N=1). An additional slot (N=2) relaxes the MAC queue to the point
$\approx$ 92\% of packets are transmitted in less than the multisuperframe duration.
Therefore, a third slot (N=3) shows a small improvement.

In general, if transmission delays depend only on the queue length, 
 deterministic communication is possible for two reasons: \one under continuous
network load, each p-value (desired quality of service) maps to a maximum queue
length, which bounds the transmission delay. \two the upper layer can remove
packets from the queue, which allows fine-grained control of the maximum
transmission delay.

